SemEval-2025 Task 3: Mu-SHROOM, the Multilingual Shared Task on Hallucinations and Related Observable Overgeneration Mistakes

We present the Mu-SHROOM shared task which is focused on detecting hallucinations and other overgeneration mistakes in the output of instruction-tuned large language models (LLMs). Mu-SHROOM addresses general-purpose LLMs in 14 languages, and frames the hallucination detection problem as a span-labeling task. We received 2,618 submissions from 43 participating teams employing diverse methodologies. The large number of submissions underscores the interest of the community in hallucination detection. We present the results of the participating systems and conduct an empirical analysis to identify key factors contributing to strong performance in this task. We also emphasize relevant current challenges, notably the varying degree of hallucinations across languages and the high annotator disagreement when labeling hallucination spans.

==> tables/participant_info/team-summary.tex <==
\rowcolors{2}{gray!25}{white}
\begin{tabular}{p{.35\linewidth} p{.25\linewidth} p{0.9\linewidth}}
    \toprule
    % \bf	Team	 \&	\bf	Paper &	\bf	Langs &	\bf	Overview		\\
    \bf	Team	 \&	\bf	Paper &	\bf	Languages &	\bf	Overview		\\
    \midrule
Advacheck \citep{voznyuk-etal-2025-advacheck} & EN & NER-based keyword extraction, wikipedia-based RAG, LLM edition-based prompting. \\
AILSNTUA \citep{karkani-etal-2025-ails} & All & translate-test (to EN and ZH) prompt-based approaches using synthetic few-shot examples. \\
ATLANTIS \citep{kobus-etal-2025-atlantis} & DE, EN, ES, FR & RAG + LLM prompting; RAG-based approaches; token-level classifiers. \\
BlueToad \citep{pronk-etal-2025-bluetoad}& AR, CS, DE, EN, ES, EU, FA, FI, FR, HI, IT, SV, ZH & QA-finetuned base PLMs; fine-tuning on synthetic data  \\
NLP\_CIMAT \citep{stack-sanchez-etal-2025-nlp_cimat} & AR, CA, CS, EN, ES, EU, FA, FI, FR, IT, SV & MLP-based classifiers probing the hidden layers of a Llama 3.1 model; few shot inference with chatGPT3.5-turbo using wikipedia contexts. \\
UZH \citep{wastl-etal-2025-uzh} & All & Prompting to generate a set of answers, using either an external model (GPT-4o-mini) or the model that produced the datapoint, followed by a prompting-based detection step to mark counterfactual spans. \\
COGUMELO \citep{creo-etal-2025-cogumelo} & EN, ES & NER-finetuning; Perplexity-based assessments \\
CUET\_SSTM & AR & NER-finetuning. \\
Team Cantharellus \citep{mo-etal-2025-team} & AR, CA, CS, DE, EN, ES, EU, FA, FI, FR, HI, IT, ZH & prompting-based approach (GPT-4o-mini) to find hallucinated words/parts of text in each datapoint; fine-tuning on synthetic data. \\
DUTJBD \citep{yin-etal-2025-dutjbd} & EN & --- \\
DeepPavlov & All & white-box approaches  \\
Deloitte \citep{chandler-etal-2025-deloitte} & All & binary token-level classifiers, trained using web-search results, task instruction and datapoint as inputs. \\
FENJI \citep{alberts-etal-2025-fenji} & All & Dense passage retrieval for Flan-T5 prompting. \\
FunghiFunghi \citep{ballout-etal-2025-funghifunghi} & EN, ES, FR, IT, SV & translate-train (to EN) and synthetic datasets. \\
GIL-IIMAS UNAM \citep{lopez-ponce-etal-2025-gil} & EN, ES & Wikipedia-based RAG. \\
Howard University - AI4PC  \citep{aryal-akomoize-2025-howard}& All & Time-series anomaly detection across the sequence of logits. \\
HalluRAG-RUG \citep{abdi-etal-2025-hallurag} & EN & Wikipeida-based RAG, followed by a summarization step and a zero-shot prompting to annotate the items. \\
HalluSearch \citep{abdallah-el-beltagy-2025-hallusearch} & All & Factual statement decomposition and verification through real-world context retrieval. \\
HalluciSeekers & AR, DE, EN, ES, FA, FR, IT, SV & --- \\
Hallucination Detectives \citep{elchafei-abu-elkheir-2025-hallucination} & AR, EN & Semantic role labeling, dependency parsing, and token-logit confidence scores to construct spans\\
HausaNLP \citep{bala-etal-2025-hausanlp} & EN & Finetuning approaches. \\
LCTeam \citep{maldonado-rodríguez-etal-2025-lcteam} & All & Label transfer via translate-train (to CA, CS, ES, FR, IT, ZH, \& between phylogenetically related languages); Wikipedia-based RAG and summarization approaches. \\
MALTO \citep{savelli-etal-2025-malto} & EN & Logits of a larger model are used to assess the truthfulness of the sentence predicted by the single smaller model. \\
NCL-UoR \citep{hong-etal-2025-ncl} & All & Keyword extraction and wikipedia-based retrieval, detection using closed-source APIs, post-processing with non-linear probability optimization or stochastic prompt-based labeling. \\
MSA \citep{hikal-etal-2025-msa} & All & Weak supervised fine-tuning approaches \\
REFIND \citep{lee-yu-2025-refind} & AR, CS, DE, EN, ES, EU, FI, FR, IT & Context sensitivity-based token-level identification matched against externally retreived documents; FAVA-based pipeline. \\
RaggedyFive \citep{heerema-etal-2025-raggedyfive} & EN & RAG + NLI across trigrams in LLM answers.  \\
S1mT5v-FMI & DE, ES, FI, FR, SV, ZH & --- \\
Swushroomsia \citep{mitrovic-etal-2025-swushroomsia}& AR, DE, EN, ES, FI, FR, HI, IT, SV, ZH & prompting-based approach \\
TU Munich & AR, DE, EN, ES, FI, FR, HI, IT, SV, ZH & Synthetic data generation (MKQA-based). \\
TUM-MiKaNi \citep{anschutz-etal-2025-tum} & All & Wikiepdia-based retrieval used as input for prompting-based approaches; BERT-based regression. \\
TrustAI & AR, DE, EN, ES, FI, FR, HI, IT, SV, ZH & variations on the neural baseline \\
UCSC \citep{huang-etal-2025-ucsc} & All & Elaborate prompting approaches (CoT, few-shot reasoning); pre-translation (to EN)  before RAG-based prompting; token masking-based approaches \\
UMUTeam \citep{pan-etal-2025-umuteam} & All & Classifier-based, compare outputs to be annotated with those from larger LLMs. \\
VerbaNexAI \citep{morillo-etal-2025-verbanexai} & EN & Retrieval-based approaches \\
YNU-HPCC \citep{chen-etal-2025-ynu}& EN, ZH & prompting, RAG; MRC. \\
CCNU \citep{liu-chen-2025-ccnu} & All & prompting \& RAG \\
iai\_MSU \citep{pukemo-etal-2025-iai_msu} & EN & RAG \\
keepitsimple \citep{vemula-krishnamurthy-2025-keepitsimple} & All & multiple llm generated responses are compared with model output text by modeling information entropy for detecting uncertainty. \\
nsu-ai & All & prompt based approaches \\ % We have more details, but my brain is too fried to make sense of this: the llm was finetuned to generate list of hallucinations during a special dialogue. the dialogue on detecting hallucinations was stopped when the model reported that it could no longer find hallucinations in the analyzed text.;the instruction token embedder with special prompt generates embeddings of answer's tokens, after that a binary classifier detects hallucinations for each of these tokens. the abovementioned special prompt contains a some world knowledge concerned with model input.;the instruction token embedder with special prompt generates embeddings of answer's tokens, after that a binary classifier detects hallucinations for each of these tokens.;this is mix of previous solutions. \\
smurfcat \citep{rykov-etal-2025-smurfcat} & All & Qwen-based approach, deriving continuous annotation through repeated sampling. \\
tsotsalab & All & GPT-4 finetuning; counterfactual comparisons with external references. \\
uir-cis \citep{huang-etal-2025-uir} & All & Comparison of extracted triples to external references. \\
\bottomrule
\end{tabular}


